ERA: Error-Resistant Autonomous Object Navigation with Predicted Depth

Depth and 3D foundation models can predict geometry from RGB images, allowing zero-shot object navigation without a depth sensor. However, when predicted depth is mapped as if it came from a sensor, view-dependent errors accumulate in the map, remove exploration goals, and end the search before the agent can observe and correct them. We propose ERA, a training-free object navigation system that replaces the depth sensor with depth predicted from RGB images and poses. ERA follows a paradigm we call Move with Error: movement provides new views that correct map errors, and the corrected map enables further movement. It realizes this paradigm with revisable occupancy and with exploration from reachable viewpoints, which continues the search when no frontier remains, and verifies the target across views before stopping. On three benchmarks, ERA achieves state-of-the-art performance among training-free methods without depth sensors. Its map and exploration components also raise VLFM's success from 10.8% to 61.7% under the same predicted depth. We further deploy ERA on a real robot.

==> tables/numbers.tex <==
\makeatletter
\expandafter\def\csname res@v1@1.0@SR\endcsname{55.2}
\expandafter\def\csname res@v1@1.0@SPL\endcsname{27.4}
\expandafter\def\csname res@v1@0.2@SR\endcsname{54.2}
\expandafter\def\csname res@v1@0.2@SPL\endcsname{27.1}
\expandafter\def\csname res@v1@0.1@SR\endcsname{53.5}
\expandafter\def\csname res@v1@0.1@SPL\endcsname{26.9}
\expandafter\def\csname res@v2@1.0@SR\endcsname{70.1}
\expandafter\def\csname res@v2@1.0@SPL\endcsname{30.6}
\expandafter\def\csname res@v2@0.2@SR\endcsname{66.3}
\expandafter\def\csname res@v2@0.2@SPL\endcsname{29.2}
\expandafter\def\csname res@v2@0.1@SR\endcsname{40.6}
\expandafter\def\csname res@v2@0.1@SPL\endcsname{17.6}
\expandafter\def\csname res@mp3d@1.0@SR\endcsname{46.4}
\expandafter\def\csname res@mp3d@1.0@SPL\endcsname{21.2}
\expandafter\def\csname res@mp3d@0.2@SR\endcsname{42.0}
\expandafter\def\csname res@mp3d@0.2@SPL\endcsname{19.1}
\expandafter\def\csname res@mp3d@0.1@SR\endcsname{39.8}
\expandafter\def\csname res@mp3d@0.1@SPL\endcsname{18.1}
\expandafter\def\csname abl@frozen@SR\endcsname{69.3}
\expandafter\def\csname abl@frozen@SPL\endcsname{29.3}
\expandafter\def\csname abl@A2S@SR\endcsname{69.8}
\expandafter\def\csname abl@A2S@SPL\endcsname{30.8}
\expandafter\def\csname abl@no_inflation@SR\endcsname{70.1}
\expandafter\def\csname abl@no_inflation@SPL\endcsname{30.6}
\expandafter\def\csname abl@A2S_plus_multiview@SR\endcsname{70.1}
\expandafter\def\csname abl@A2S_plus_multiview@SPL\endcsname{30.6}
\makeatother

